Low-Stack HAETAE for Memory-Constrained Microcontrollers

We present a low-stack implementation of the module-lattice signature scheme HAETAE, targeting microcontrollers with 8 kB-16 kB of available SRAM. On such devices, peak stack usage is often the binding constraint, and HAETAE's hyperball-based sampler, large transient polynomial vectors, and variable-length signature payloads (hint and high-bits arrays) pose a particular challenge. To address this we introduce (i) Rejection-aware pass decomposition, which isolates encoding to the post-acceptance path; (ii) Component-level early rejection, which short-circuits the response computation when a partial norm already exceeds the bound; and (iii) Reverse-order streaming entropy coding using range Asymmetric Numeral Systems (rANS), which eliminates full hint and high-bits staging buffers. Combined with streamed matrix generation, a two-pass hyperball sampler with streaming Gaussian backend, and row-streamed verification, these techniques bring Signing stack from 71 kB-141 kB in the reference implementation down to 5.8 kB-6.0 kB, key generation to 4.7 kB-5.7 kB, and verification to 4.7 kB-4.8 kB across all three security levels. Our pure C implementation covers all three security levels (HAETAE-2/3/5), whose optimization paths differ due to the public-key domain (d>0 vs. d=0) and rejection structure. We implement our optimization on a Nucleo-L4R5ZI and compare to the reference pqm4 (for HAETAE-2 and -3) and a recently published memory-optimized implementation (targeting HAETAE-5 only). We reduce HAETAE-2, -3, and -5 stack by respectively 75, 86 and 8 % for key generation, 92, 95 and 24 % for signature generation, and 85, 91 and 22 % for verification. Depending on the parameter set, this impacts performance by at most a factor 1.8 and 3.4 for key and signature generation respectively, while even offering a performance improvement up to 18 % for verification. Verification at all security levels fits within 8 kB of RAM (signature buffer + stack) and is 2.34-3.34x faster than ML-DSA m4fstack at each comparable security level. We additionally validate portability under RIOT-OS on ARM Cortex-M4 and RISC-V targets.

==> improved.tex <==
\section{Low-footprint implementation and results}
\label{sec:impl:results}

This section summarizes the implementation choices that allow \hae to run on
constrained Cortex-M class devices, and reports the resulting stack
footprints for \hae-120 (mode 2, with $N=256$, $K=2$, $L=4$).

\paragraph{Build configuration.}
Unless stated otherwise, we compile with size optimization and the following
memory-saving options enabled:
\begin{center}
\texttt{-Os -DSTREAM\_MATRIX=1 -DFROZEN\_A=1 -DSAMPLER=2}.
\TODO{YB: i updated -DFROZEN\_A = 2 which streams the matrix coefficients instead of storing frozend polynomial with static memory.}
\end{center}
Here, \texttt{STREAM\_MATRIX} regenerates matrix entries on demand,
\texttt{FROZEN\_A} keeps the expanded matrix in a compact (seed/nonce driven)
representation, and \texttt{SAMPLER=2} selects the two-pass streamed hyperball
sampler from Section~\ref{sec:sampler}.

\paragraph{Stack profiling methodology.}
We use a high-watermark technique: the full stack region is initialized with a
canary pattern at startup, and each labeled scope scans for the deepest
overwrite. We report the maximum stack consumption within each scope and for
the overall \texttt{keypair}, \texttt{sign}, and \texttt{verify} routines.

\paragraph{Results.}
Table~\ref{tab:stack-haetae120} reports the measured peak stack usage.
For \hae-120, both key generation and signing fit within \SI{16}{\kilo\byte} of
stack, and our low-stack verification now fits within \SI{15}{\kilo\byte}.
(For reference, the same verification refactoring reduces \hae-256 (mode~5) to
\SI{17.7}{\kilo\byte} peak stack on Cortex-M4, at the cost of additional
recomputation.)

\begin{table}[t]
  \centering
  \caption{Peak stack usage (bytes) for \hae-120 on Cortex-M4 with
  \texttt{-Os -DSTREAM\_MATRIX=1 -DFROZEN\_A=1 -DSAMPLER=2}.}
  \label{tab:stack-haetae120}
  \begin{tabular}{lrr}
    \toprule
    Scope & Base [B] & Peak [B] \\
    \midrule
    \texttt{keypair}                   & 4\,024 & 15\,592 \\
    \texttt{sign:passA\_challenge}     & 5\,528 & 10\,084 \\
    \texttt{sign:passB\_z\_and\_check} & 5\,528 &  7\,916 \\
    \texttt{sign:passC\_hint\_pack}    & 5\,528 &  9\,516 \\
    \texttt{sign}                      & 4\,024 &  9\,516 \\
    \texttt{verify}                    & 4\,024 & 14\,452 \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Where the savings come from.}
The reductions follow the Bos--Renes--Sprenkels playbook: (i) stream objects
derived from seeds instead of materializing them; (ii) tightly scope
temporaries so large buffers do not overlap; and (iii) recompute cheap values
instead of storing them across rejection loops. Concretely, our implementation
streams matrix generation in key generation and signing, uses a two-pass
sampler to avoid storing Gaussian samples, performs sparse challenge
multiplication without NTT buffers, and packs directly into the signature
buffer to avoid intermediate encoding arrays; verification is refactored into a
row-streamed pipeline that reuses a constant-size workspace.

\subsection{Row-streamed verification}
\label{sec:impl:verify-rowstream}

Our largest savings in verification come from a \emph{row-streamed} refactoring
in the spirit of Bos--Renes--Sprenkels: rather than materializing the full
intermediate vectors $\mathbf t \in \Rq^{K}$, $\mathbf w \in \Rq^{K}$, and
$\mathbf z_2 \in \Rq^{K}$ on the stack, we process one output row at a time and
immediately fold it into the challenge transcript.

\paragraph{High-level structure.}
Given a public key $\pk=(\rho,\mathbf b)$ and a signature
$\sigma=(\mathbf c,\mathrm{LB}(\mathbf z_1),\mathrm{HB}(\mathbf z_1),\mathbf h)$
(in compressed form), verification recomputes the challenge $\mathbf c'$ from a
transcript that depends on $\mathrm{HB}(\mathbf w)$ and $\mathbf w'$.
The refactored verification proceeds as follows:
\begin{enumerate}
  \item \textbf{View-style parsing.} We keep $\mathrm{LB}(\mathbf z_1)$ as a
  pointer into the signature buffer, decode only $\mathrm{HB}(\mathbf z_1)$
  into an \texttt{int8} array, and decode $\mathbf h$ into a compact
  \texttt{uint16} array. In addition, we represent $\mathbf w' \in \mathcal{R}_2$
  as a packed bitstring of $N/8$ bytes.
  \item \textbf{Pre-pass.} In a single sweep over the coefficients, we
  (re)compose each coefficient of $\mathbf z_1$ on-the-fly as
  $z = 2^8 \cdot \mathrm{HB}(z) + \mathrm{LB}(z)$, accumulate
  $\lVert\mathbf z_1\rVert_2^2$, and compute the packed bits of
  $\mathbf w' = \mathrm{LSB}(\mathbf z_1^{(0)} - \mathbf c)$.
  \item \textbf{Row-streamed product and transcript.} For each row
  $r \in \{0,\dots,K-1\}$, we recompute the NTT-domain accumulator
  \[
    t_r \;\gets\; \sum_{\ell=0}^{L-1} A_{1}[r,\ell] \cdot \ntt(z_{1,\ell}),
  \]
  by (re)composing and transforming one column $z_{1,\ell}$ at a time and
  streaming $A_1[r,\ell]$ from $\rho$. After an inverse NTT, we reconstruct the
  mod-$2q$ representative via CRT (using $\mathbf w'$ for $r=0$), compute
  $w_r \gets \mathrm{HB}(t_r) + h_r$, and immediately pack
  $\mathrm{HB}(w_r)$ into the transcript buffer.
  \item \textbf{Incremental norm check.} Still within the row loop, we recover
  \(z_{2,r} \gets (\alpha w_r - t_r + w'_r)/2 \bmod q\) and accumulate
  $\lVert z_{2,r}\rVert_2^2$, aborting early as soon as
  $\lVert\mathbf z_1\rVert_2^2 + \lVert\mathbf z_2\rVert_2^2 > B_2^2$.
  \item \textbf{Re-derive the challenge.} Finally, we hash the packed
  transcript $(\mathrm{HB}(\mathbf w),\mathbf w')$ together with
  $\mu = H(\pk\cc m)$ to recompute $\mathbf c'$, and compare it bitwise to the
  $\mathbf c$ embedded in the signature.
\end{enumerate}

\paragraph{Why this reduces peak stack.}
In the reference verifier, several large vectors are live simultaneously:
decoded $\mathbf z_1$ (or its parts), the product vector $\mathbf t$, the
high-bits vector $\mathbf w$, the recovered $\mathbf z_2$, and temporary
decoding buffers.
Row-streaming reduces the liveness to a constant-size working set: three
polynomials (a precomputed first-column entry derived from $\mathbf b$, a
per-row accumulator, and a reused $z$ scratch), two compact decoded arrays
($\mathrm{HB}(\mathbf z_1)$ and $\mathbf h$), and the packed transcript.
This removes the need for multiple concurrent \texttt{polyveck} allocations and
is what drives the verification peak down to \SI{14.5}{\kilo\byte} for
\hae-120 and \SI{17.7}{\kilo\byte} for \hae-256 on Cortex-M4.

\paragraph{Tradeoff.}
The price of row-streaming is recomputation: each output row reprocesses the
$L$ columns of $\mathbf z_1$ (including $L$ NTTs), roughly multiplying the
matrix--vector work by a factor $K$. In our target setting (minimal SRAM on
Cortex-M devices), this time--memory tradeoff is acceptable.


==> origin_eval.tex <==
\section{Benchmark \& Evaluation}


\begin{table*}[t]

\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
% Column widths sum to ~1.00\linewidth
\begin{tabular}{
  p{0.13\linewidth}
  p{0.10\linewidth}
  p{0.17\linewidth}
  p{0.13\linewidth}
  p{0.16\linewidth}
  p{0.16\linewidth}
  p{0.14\linewidth}
}
\toprule
Variant & Build & Knobs & Memory & Key generation & Signing & Verification \\
\midrule

\textbf{HAETAE-2} & Baseline &
\texttt{SAMPLER=1}\newline
\texttt{STREAM=0}\newline
\texttt{FROZEN=0} &
Flash: --\newline
SRAM: -- &
Stack: \num{5280}$\rightarrow$\num{17356}\newline
$\Delta$=\num{12076}\newline
Cycles: \num{7823181} &
Stack: \num{5280}$\rightarrow$\num{52412}\newline
$\Delta$=\num{47132}\newline
Cycles: \num{39511183} &
Stack: \num{5280}$\rightarrow$\num{23616}\newline
$\Delta$=\num{18336}\newline
Cycles: \num{1457363} \\
\cline{2-7}
& Low-stack &
\texttt{SAMPLER=2}\newline
\texttt{STREAM=1}\newline
\texttt{FROZEN=2} &
Flash: \num{83756}~B\newline
SRAM: \num{13148}~B &
Stack: \num{4032}$\rightarrow$\num{10412}\newline
$\Delta$=\num{6380}\newline
Cycles: \num{10231926} &
Stack: \num{4032}$\rightarrow$\num{10016}\newline
$\Delta$=\num{5984}\newline
Cycles: \num{189807771} &
Stack: \num{4032}$\rightarrow$\num{14472}\newline
$\Delta$=\num{10440}\newline
Cycles: \num{1494650} \\
\midrule

\textbf{HAETAE-3} & Baseline &
\texttt{SAMPLER=1}\newline
\texttt{STREAM=0}\newline
\texttt{FROZEN=0} &
Flash: --\newline
SRAM: -- &
Stack: \num{7352}$\rightarrow$\num{22580}\newline
$\Delta$=\num{15228}\newline
Cycles: \num{16588394} &
Stack: \num{7352}$\rightarrow$\num{75052}\newline
$\Delta$=\num{67700}\newline
Cycles: \num{11889733} &
Stack: \num{7352}$\rightarrow$\num{32096}\newline
$\Delta$=\num{24744}\newline
Cycles: \num{2858628} \\
\cline{2-7}
& Low-stack &
\texttt{SAMPLER=2}\newline
\texttt{STREAM=1}\newline
\texttt{FROZEN=2} &
Flash: \num{83788}~B\newline
SRAM: \num{17244}~B &
Stack: \num{6104}$\rightarrow$\num{12492}\newline
$\Delta$=\num{6388}\newline
Cycles: \num{17535485} &
Stack: \num{6104}$\rightarrow$\num{13400}\newline
$\Delta$=\num{7296}\newline
Cycles: \num{231115813} &
Stack: \num{6104}$\rightarrow$\num{20416}\newline
$\Delta$=\num{14312}\newline
Cycles: \num{2790930} \\
\midrule

\textbf{HAETAE-5} & Baseline &
\texttt{SAMPLER=1}\newline
\texttt{STREAM=0}\newline
\texttt{FROZEN=0} &
Flash: --\newline
SRAM: -- &
Stack: \num{8780}$\rightarrow$\num{22572}\newline
$\Delta$=\num{13792}\newline
Cycles: \num{18213558} &
Stack: \num{8780}$\rightarrow$\num{90484}\newline
$\Delta$=\num{81704}\newline
Cycles: \num{57072317} &
Stack: \num{8780}$\rightarrow$\num{37620}\newline
$\Delta$=\num{28840}\newline
Cycles: \num{3788664} \\
\cline{2-7}
& Low-stack &
\texttt{SAMPLER=2}\newline
\texttt{STREAM=1}\newline
\texttt{FROZEN=2} &
Flash: \num{82660}~B\newline
SRAM: \num{20316}~B &
Stack: \num{7944}$\rightarrow$\num{15476}\newline
$\Delta$=\num{7532}\newline
Cycles: \num{13040301} &
Stack: \num{7944}$\rightarrow$\num{16180}\newline
$\Delta$=\num{8236}\newline
Cycles: \num{261546804} &
Stack: \num{7944}$\rightarrow$\num{17672}\newline
$\Delta$=\num{9728}\newline
Cycles: \num{4371330} \\
\bottomrule
\end{tabular}

\caption{Evaluation on STM32F411E-DISCO. Stack is reported as base$\rightarrow$peak within the operation (and $\Delta$). Memory is static footprint (Flash/SRAM).}
\label{tab:haetae-f411-eval}
\end{table*}

tools: arm-none-eabi-gcc (Arch Repository) 14.2.0


\paragraph{Footprint metrics.}
We report the static code and memory footprint using 
\texttt{arm-none-eabi-size} in Berkeley format.
The \texttt{text} field accounts for executable code and 
read-only data mapped to Flash, while \texttt{data} is the 
initialized data section stored in Flash but copied to RAM at 
boot, and \texttt{bss} is the zero-initialized data section 
residing in RAM.
Accordingly, we estimate Flash usage as $\texttt{text}+\texttt{data}$ 
and static SRAM usage as $\texttt{data}+\texttt{bss}$.
These footprint numbers exclude the runtime stack, which we measure 
separately.
For stack usage, ``base$\rightarrow$peak'' reports the stack 
consumption at scope entry (base) and the maximum observed within 
the operation (peak); $\Delta$ is the additional stack required by 
the operation beyond the baseline.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}

